ANNETTE: Accurate Neural Network Execution Time Estimation with Stacked Models

With new accelerator hardware for DNN, the computing power for AI applications has increased rapidly. However, as DNN algorithms become more complex and optimized for specific applications, latency requirements remain challenging, and it is critical to find the optimal points in the design space. To decouple the architectural search from the target hardware, we propose a time estimation framework that allows for modeling the inference latency of DNNs on hardware accelerators based on mapping and layer-wise estimation models. The proposed methodology extracts a set of models from micro-kernel and multi-layer benchmarks and generates a stacked model for mapping and network execution time estimation. We compare estimation accuracy and fidelity of the generated mixed models, statistical models with the roofline model, and a refined roofline model for evaluation. We test the mixed models on the ZCU102 SoC board with DNNDK and Intel Neural Compute Stick 2 on a set of 12 state-of-the-art neural networks. It shows an average estimation error of 3.47% for the DNNDK and 7.44% for the NCS2, outperforming the statistical and analytical layer models for almost all selected networks. For a randomly selected subset of 34 networks of the NASBench dataset, the mixed model reaches fidelity of 0.988 in Spearman's rank correlation coefficient metric. The code of ANNETTE is publicly available at https://github.com/embedded-machine-learning/annette.

==> sections/future_work.tex <==


\section{Future Work}

\begin{itemize}
\item @MixedModels: it would be interesting to pack it all in a model
\subitem One model with polynomial components and components for the tiles
\subitem Automatically detect the points of interest
\subitem Since these points occur periodically we could try and fit some kind of wave and amplitude and frequency is the modelling parameter
\subitem at first subtract to generate an overall smoother surface.
\subitem random measurements to find the optimal points and then derive the best parameter settings for $S_i$
\subitem comparison between estimating gops and time what works better and mathematical background?
\item @MixedModels: it would be interesting to better automate the whole process
\item @MixedModels: add terms for memory effects to find where the stuff from NCS2 comes from
\item @Statistical Models: there should be an expression or steps also for the Memory Borders. How can we efficiently determine those.
\item @Statistical Models: It would be cool to have the statistical model so far parametric that for similar architectures you can use one characterization to know what will happen in another

\item @Graph Optimized: Make a more sophisticated optimizer estimation thingy
\item @Determining $S_i$ and $\alpha$ with help of decision trees


\end{itemize}


==> sections/pre.tex <==
\newpage
\section{General thoughts not to put in paper}

\subsection{Selected Hardware}
\begin{itemize}
    \item NCS2 (NPU)
    \item DNNDK (FPGA)
    %\item Cesar (Siemens FPGA HLS Design)
\end{itemize}

\subsection{Modeling Layer Optimizations}
\begin{itemize}
    \item Hardware Independent Optimizations
    \item Hardware Specific Optimizations
    \begin{itemize}
        \item Fuse Convolution+Pooling
        \item Fuse Activation
    \end{itemize}
\end{itemize}


\subsection{Datapoint selection}
\begin{itemize}
    \item it is import to vary all of the parameters and select a meaningful dataset
    \item for the sake of prediction the larger layers with larger execution time are more important therefore the error should possibly be selected as mean average error better than mean average percentage error
\end{itemize}

\section{LayerTypes done}
\begin{itemize}
    \item 1x1 Conv, 3x3 Conv, 5x5 Conv, 7x7 Conv + 2x2 Pool
    \item 1x1 Conv, 3x3 Conv, 5x5 Conv, 7x7 Conv + 2x2 Pool
    \item 1x1 Conv, 3x1 Conv, 5x1 Conv, 7x1 Conv 
\end{itemize}

\section{LayerTypes todo}
\begin{itemize}
    \item nonsymmetrical Conv 1x7, 7x1 (Inception Net)
    \item 3x3 Pooling (Inception Net, NASBench Nets)
    \item Fully Connected 2048x1000 (Inceptionv3)
    \item 3x3 Pooling Average (Inception Net)
    \item Global Pool 8x8 (Inceptionv3)
    \item Concatenate Layer (Estimation and Optimization) (Inceptionv1)
\end{itemize}

\section{Observations}
\begin{itemize}
    \item reduce on realistic use cases to reduce data we need to collect
    \item important features are overall operations and also amount of input and output data
    \item Test on real network data to verify if realistic
    \item imbalanced dataset due to selection of data, this make be a problem for the predictor
    \item seems like bad hardwaresupport for higher stride
\end{itemize}

\section{DNNDK}
\begin{itemize}
    \item Fuses most layers therefore difficult to measure each layer separately
    \item careful what you are measuring
\end{itemize}

\section{NCS2}
\begin{itemize}
    \item Fuses most layers therefore difficult to measure each layer separately
    \item careful what you are measuring
\end{itemize}


%\begin{table}[ht]
%    \centering
%    \caption{Performed microkernel benchmarks}
%    \label{tab:mk_benchmarks}
%    \begin{tabular}{l|l|l}
%     \hline
%     layer type & parameters & datapoints \\ 
%     \hline
%     \hline
%     Conv2D square (sq.) & h, w, c, f, kernel\_size & 35000 %\\  
%     Conv2D 1xw & h, w, c, f, kernel\_width & 35000 \\
%     Conv2D hx1 & h, w, c, f, kernel\_height & 35000\\
%     Conv2D sq. stride 2 & h, w, c, f, kernel\_size & 35000 %\\  
%     DWSepConv2D sq. & h, w, c, kernel\_size & 1000\\
%     MaxPool sq. & h, w, c, kernel\_size, stride & 1000\\
%     AvgPool sq. & h, w, c, kernel\_size, stride & 1000\\
%     Fully Connected & c, f & 500\\
%     Conv2D sq. pool 2x2 & h, w, c, f, kernel\_size & 35000 %\\  
%     Conv2D sq. pool 3x3 & h, w, c, f, kernel\_size & 35000 %\\  
%     DwSConv sq.+ Conv2D 1x1 & h, w, c, f, kernel\_size & %35000\\
%     \hline
%    \end{tabular}
%\end{table}


\section{Related work i found so far}


